A simple normative network approximates local non-Hebbian learning in the cortex

To guide behavior, the brain extracts relevant features from high-dimensional data streamed by sensory organs. Neuroscience experiments demonstrate that the processing of sensory inputs by cortical neurons is modulated by instructive signals which provide context and task-relevant information. Here, adopting a normative approach, we model these instructive signals as supervisory inputs guiding the projection of the feedforward data. Mathematically, we start with a family of Reduced-Rank Regression (RRR) objective functions which include Reduced Rank (minimum) Mean Square Error (RRMSE) and Canonical Correlation Analysis (CCA), and derive novel offline and online optimization algorithms, which we call Bio-RRR. The online algorithms can be implemented by neural networks whose synaptic learning rules resemble calcium plateau potential dependent plasticity observed in the cortex. We detail how, in our model, the calcium plateau potential can be interpreted as a backpropagating error signal. We demonstrate that, despite relying exclusively on biologically plausible local learning rules, our algorithms perform competitively with existing implementations of RRMSE and CCA.

==> figures/cca_circuit.tex <==
\begin{tikzpicture}
    %x inputs
    \coordinate (a1) at (0,0);
    \coordinate[right=6.4cm of a1] (a1R);
    \path[-, thick,  black!10!red] (a1) edge (a1R);
    \coordinate[above=.2cm of a1] (a2);
    \coordinate[right=6.4cm of a2] (a2R);
    \path[-, thick,  black!10!red] (a2) edge (a2R);
    \node[ainput] at ($(a1)!0.5!(a2)$) {${\y}$};

    %pyramidal neurons
    \node[zneuron, below right=1.9cm and 1.2cm of a1] (z1) {};
    \node at (z1) {$z_1$};
    \node[zneuron, right=2.2cm of z1] (zd) {};
    \node at (zd) {$z_k$};
    \node at ([yshift=-0cm]$(z1)!0.5!(zd)$) (zdots) {$\cdots$};
    \node[apical, above=2.2cm of z1] (z1A) {};
    \node[apical, above=2.2cm of zd] (zdA) {};
    
    \path[thick] (z1) edge (z1A);
    \path[thick] (zd) edge (zdA);
    
    %y inputs
    \coordinate[below=2.9cm of a1] (b1);
    \coordinate[right=6.4cm of b1] (b1R);
    \path[-, white!10!blue, thick] (b1) edge (b1R);
    \coordinate[below=.2cm of b1] (b2);
    \coordinate[right=6.4cm of b2] (b2R);
    \path[-, white!10!blue, thick] (b2) edge (b2R);
    \coordinate[below=.2cm of b2] (b3);
    \coordinate[right=6.4cm of b3] (b3R);
    \path[-, white!10!blue, thick] (b3) edge (b3R);
    \node[binput] at (b2) {${\x}$};

    %interneuron
    \coordinate[below left=-2.0cm and 0.75cm of b1R] (i1);
    \coordinate[left=5.95cm of i1] (i1R);
    \coordinate[above right=.2cm and .2cm of i1] (i2);
    \coordinate[above=.2cm of i1R] (i2R);
    % \coordinate[below right=.2cm and .2cm of i2] (i3);
    % \coordinate[below=.2cm of i2R] (i3R);

    \coordinate[below=3.3cm of i1] (int1N);
    \coordinate[right=.2cm of int1N] (int2N);
    % \coordinate[right=.2cm of int2N] (int3N);
    % \node[ineuron] at (int3N) (int3) {};
    \node[ineuron] at (int2N) (int2) {};
    \node[ineuron] at (int1N) (int1) {$\n$};
    
    \draw[-stealth,  black!30!green, thick] (int1) -- (i1) -- (i1R);
    \draw[-stealth,  black!30!green, thick] (int2) -- (i2) -- (i2R);
    % \draw[-stealth,  black!30!green, thick] (int3) -- (i3) -- (i3R);

    %apical synapses
    %\node[above left=1cm and .3cm of z1A] (z1A1) {};
    %\path[-, thick] (z1A) edge (z1A1);
    %\node[above right=1cm and .3cm of z1A] (z1A2) {};
    %\path[-, thick] (z1A) edge (z1A2);
    \node[asynapse] at (intersection of z1--z1A and a2--a2R) {};
    \node[asynapse] at (intersection of z1--z1A and a1--a1R) (as1) {};
    % \node[below left=-.01cm and -.1cm of as1] {${\color{red}a_1}$};

    %\node[above left=1cm and .3cm of zdA] (zdA1) {};
    %\path[-, thick] (zdA) edge (zdA1);
    %\node[above right=1cm and .3cm of zdA] (zdA2) {};
    %\path[-, thick] (zdA) edge (zdA2);
    \node[asynapse] at (intersection of zd--zdA and a2--a2R) {};
    \node[asynapse] at (intersection of zd--zdA and a1--a1R) (asd) {};
    % \node[below left=-.01cm and -.1cm of asd] {${\color{red}a_k}$};

    %axon
    \coordinate[below=2.45cm of z1] (z1Axon) {};
    \coordinate[below=2.25cm of zd] (zdAxon) {};

    \coordinate[right=4.85cm of z1Axon] (pyA1);
    \coordinate[above=.2cm of pyA1] (pyA2);
    
    \draw[-stealth, very thick] (z1) -- (z1Axon) -- (pyA1);
    \draw[-stealth, very thick] (zd) -- (zdAxon) -- (pyA2);
    
    %basal synapses
    % \node[below left=1.0cm and .5cm of z1] (z1B1) {};
    % \path[-, thick] ([xshift=-.25cm] z1.south west) edge (z1B1);
    \node[below left=1.0cm and .2cm of z1] (z1B2) {};
    \path[-, thick] ([xshift=-.25cm] z1.south west) edge (z1B2);
    \node[bsynapse] at (intersection of [xshift=-.25cm] z1.south west--z1B2 and b3--b3R) {};
    \node[bsynapse] at (intersection of [xshift=-.25cm] z1.south west--z1B2 and b2--b2R) {};
    \node[bsynapse] at (intersection of [xshift=-.25cm] z1.south west--z1B2 and b1--b1R) (bs1) {};
    % \node[above left=.01cm and -.15cm of bs1] {${\color{blue}b_1}$};

    \node[below left=1.0cm and .2cm of zd] (zdB1) {};
    \path[-, thick] ([xshift=-.25cm] zd.south west) edge (zdB1);
    % \node[below left=1.0cm and .5cm of zd] (zdB2) {};
    % \path[-, thick] ([xshift=-.25cm] zd.south west) edge (zdB2);
    \node[bsynapse] at (intersection of [xshift=-.25cm] zd.south west--zdB1 and b3--b3R) {};
    \node[bsynapse] at (intersection of [xshift=-.25cm] zd.south west--zdB1 and b2--b2R) {};
    \node[bsynapse] at (intersection of [xshift=-.25cm] zd.south west--zdB1 and b1--b1R) (bsk) {};
    % \node[above left=.01cm and -.15cm of bsk] {${\color{blue}b_k}$};

    %\node[below right=0.9cm and .2cm of z1] (z1I1) {};
    %\path[-, thick] ([xshift=.25cm] z1.south east) edge (z1I1);
    % \node[below right=1.8cm and -.15cm of z1] (z1I2) {};
    % \path[-, thick] ([xshift=.25cm] z1.south east) edge (z1I2);
    % \node[isynapse] at (intersection of [xshift=.25cm] z1.south east--z1I2 and i3--i3R) {};
    \node[isynapse] at (intersection of  z1--z1A and i2--i2R) {};
    \node[isynapse] at (intersection of  z1--z1A and i1--i1R) {};
    
    
    %\node[bsynapse] at (intersection of [xshift=.25cm] z1.south east--z1I1 and b2--b2R) {};

    % \node[below right=1.0cm and .45cm of zd] (zdI1) {};
    % \path[-, thick] ([xshift=.25cm] zd.south east) edge (zdI1);
    %\node[below right=1.0cm and .2cm of zd] (zdI2) {};
    %\path[-, thick] ([xshift=.25cm] zd.south east) edge (zdI2);
    % \node[isynapse] at (intersection of [xshift=.25cm] zd.south east--zdI2 and i3--i3R) {};
    \node[isynapse] at (intersection of zd--zdA and i2--i2R) {};
    \node[isynapse] at (intersection of zd--zdA and i1--i1R) {};
    %\node[bsynapse] at (intersection of [xshift=.25cm] zd.south east--zdI2 and b2--b2R) {};
    
    %axon to interneuron
    \node[below left=0.8cm and -.25cm of int1] (int1S) {};
    \node[below right=0.8cm and -.25cm of int2] (int2S) {};
    % \node[below right=0.9cm and -.15cm of int3] (int3S) {};
    
    \path[-,  black!30!green, thick] (int1.south) edge (int1S);
    \path[-,  black!30!green, thick] (int2.south) edge (int2S);
    % \path[-,  black!30!green, thick] (int3.south) edge (int3S);

    \node[psynapse] at (intersection of int1.south--int1S and z1Axon--pyA1) {};
    \node[psynapse] at (intersection of int1.south--int1S and zdAxon--pyA2) {};
    \node[psynapse] at (intersection of int2.south--int2S and z1Axon--pyA1) {};
    \node[psynapse] at (intersection of int2.south--int2S and zdAxon--pyA2) {};
    % \node[psynapse] at (intersection of int3.south--int3S and z1Axon--pyA1) {};
    % \node[psynapse] at (intersection of int3.south--int3S and zdAxon--pyA2) {};
    
    \node[asynapse] at (2.15,-4.0) (p) {}; 
    \node[right=0.07cm of p] (atext) {\scriptsize $\!\V_{\!y}^\top$};
    \node[psynapse] at (2.15,-4.4) (a) {};
    \node[right=0.07cm of a] (ptext) {\scriptsize $\Q$};
    \node[bsynapse] at (3.3,-4.0) (b) {};
    \node[right=0.07cm of b] (btext) {\scriptsize $\!\V_{\!x}^\top\!$};
    \node[isynapse] at (3.3,-4.4) (i) {};
    \node[right=0.07cm of i] (itext) {\scriptsize $\!\!\Q^\top\!$};
    \draw[rounded corners=0.2,color=black!50] (1.9,-3.785) rectangle (4.1,-4.605);
\end{tikzpicture}

==> sections/problem_statement.tex <==

In this section, we review the Reduced-Rank Regression~(RRR) problem which encompasses Canonical Correlation Analysis (CCA) and Reduced Rank (minimum) Mean Square Error (RRMSE) as special cases.

\paragraph{Notation.~} For positive integers $m,n$, let $\R^m$ denote $m$-dimensional Euclidean space, and let $\R^{m\times n}$ denote the set of $m\times n$ real-valued matrices. 
We use boldface lower-case letters (e.g., $\v$) to denote vectors and boldface upper-case letters (e.g., $\M$) to denote matrices.
Let $\I_m$ denote the $m\times m$ identity matrix.

Let $\{(\x_t,\y_t)\}_{t=1}^T$ be a sequence of pairs of data points with $\x_t\in\R^m,\;\y_t\in\R^n$.
We refer to $\x_t$ as the predictor variable and $\y_t$ as the response variable.
Define the data matrices $\X:=[\x_1,\dots,\x_T]\in\R^{m\times T}$ and $\Y:=[\y_1,\dots,\y_T]\in\R^{n\times T}$.
Let $\C_{xx}:=\tfrac1T\X\X^\top$, $\C_{yy}:=\tfrac1T\Y\Y^\top$, and $\C_{xy}:=\tfrac1T\X\Y^\top$ be the empirical covariance matrices.
Throughout this paper, we assume that $\X$ and $\Y$ are centered and full rank.

\subsection{Problem formulation~} 
The goal of RRR is to find a low-rank projection matrix $\P\in\R^{n\times m}$ that minimizes the error between $\P\X$ and $\Y$. 
The low-rank constraint favors  the extraction of features that are most predictive of the response variables, thus preventing over-fitting ~\cite{rrr_book}.
We can formalize this as follows:
% Let $\C_{xy}:=\tfrac1T\X\Y^\top$ be the empirical covariance matrix.
% Consider the generalized regression problem
\begin{align}
\label{eq:genrrr}
    \argmin{{\bf P}\in\R^{n\times m}} \frac1T\big\lVert \Y-\P\X \big\rVert_\Sigma^2 \quad\text{subject to}\quad\text{rank}(\P)\le k,
\end{align}
where $k\le\min(m,n)$ determines the rank of the problem, $\Sig\in\R^{n\times n}$ is a positive definite matrix, and $\|\cdot\|_\Sigma$ is the $\Sig$-norm defined by $\|\A\|^2_\Sigma:=\tr\A^\top\Sig\A$ for $\A\in\R^{n\times T}$.
%$\big\lVert \Y-\P\X \big\rVert_\Sigma^2 $ is the $\Sig$-norm of $(\Y-\P\X)$ defined as
% \begin{equation*}
%     \big\lVert \Y-\P\X \big\rVert_\Sigma^2 := \tr(\Y-\P\X)^\top\Sig(\Y-\P\X).
% \end{equation*}
Intuitively, the $\Sig$-norm is a generalized norm that can take into account the noise statistics of the samples~\cite{mahalanobis}. 
Two common choices for $\Sig$ are $\Sig=\I_n$ and $\Sig=\C_{yy}^{-1}$. 
When $\Sig=\I_n$, the RRR problem reduces to minimizing the mean square error (MSE) with a low-rank constraint. We refer to this objective as Reduced Rank (minimum) Mean Square Error (RRMSE)~\cite{rrr_book}.\footnote{Also referred to as reduced rank Wiener filter or simply reduced rank regression.} 
For $\Sig=\C_{yy}^{-1}$, the objective in Eq.~\eqref{eq:genrrr} is equivalent to Canonical Correlation Analysis (CCA)~(see Sec.~\ref{app:CCA_from_grrr} of the supplementary materials).
% For a more detailed discussion of the relationship of CCA with the reduced rank regression task and intuitive interpretation see Sec.~\ref{app:CCA_from_grrr} of the supplementary materials.
% with $\Sig\in\R^{n\times n}$ a positive definite matrix (see e.g. \cite[Chapter 2.1]{rrr_book}).
% which defines the optimization norm

%  that normalizes the error between $\Y$ and $\P\X$. 
% The objective function in Eq.~\eqref{eq:genrrr} is closely related to many popular dimensionality reduction techniques in statistics \cite{izenman1975reduced}.
% For example:
% \begin{itemize}
%     \item When $\Y=\X$ and $\Sig=\I_n$, then this is an objective function for PCA.
%     \item When $\Sig=\I_n$ and $\P$ is full rank, this is usual linear regression.
%     \item When $\Sig=\C_{yy}$, this is CCA.
% \end{itemize}
 %for the historical background of the objective function in Eq.~\eqref{eq:genrrr}.

\subsection{Parametrizing the projection matrix}

The low-rank constraint, $\text{rank}(\P)\le k$, in Eq.~\eqref{eq:genrrr} can be enforced by expressing $\P=\Sig^{-1}\V_y\V_x^\top$, where $\V_x\in\R^{m\times k}$ and $\V_y\in\R^{n\times k}$ (the inclusion of $\Sig^{-1}$ here is for convenience in the derivation below).
The matrix $\V_x^\top$ projects the inputs $\x_t$ onto a $k$-dimensional subspace and the column vectors of $\Sig^{-1}\V_y$ span the range of the projection matrix $\P$. 
Plugging into Eq.~\eqref{eq:genrrr}, we have
\begin{align}
\label{eq:genrrr1}
    \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}} \frac1T\big\lVert \Y-\Sig^{-1}\V_y\V_x^\top\X \big\rVert_\Sigma^2. 
    % = \Tr(\Y-\Sig^{-1}\V_y\V_x^\top\X)^\top\Sig^{-1}(\Y-\Sig\V_y\V_x^\top\X).
\end{align}
The minimum of this objective is not unique: given a solution $(\V_x,\V_y)$ and any invertible matrix $\M\in\R^{k\times k}$, $(\V_x\M^\top,\V_y\M^{-1})$ is also a solution. 
To constrain the solution set, we impose the whitening constraint $\V_x^\top\C_{xx}\V_x=\I_k$.
Expanding the quadratic in \eqref{eq:genrrr1}, dropping terms that do not depend on $\V_x$ or $\V_y$, and using the whitening constraint, we arrive at
% the following optimization problem:
\begin{align}\label{eq:genrrr2}
    \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\Tr(\V_y^\top\Sig^{-1}\V_y-2\V_x^\top\C_{xy}\V_y)\quad\text{subject to}\quad\V_x^\top\C_{xx}\V_x=\I_k.
\end{align}
% This objective function will be used for the derivation of our algorithms in the following section. 
The output of our algorithms will be the low-rank projection of $\X$, which we call $\Z:=\V_x^\top \X$. Intuitively, for RRMSE ($\Sig = \I_n$), optimization of this objective would find $\Z$ which is most informative, in terms of MSE loss, of the response variable $\Y$. 
For CCA ($\Sig = \C_{yy}^{-1}$), optimization of this objective finds the projection $\Z$ which has the highest correlation with the response variable $\Y$. 

We parametrize the normalizing matrix by its inverse as $\Sig^{-1} = \Sig_s^{-1}:= s\,\C_{yy}  + (1-s)\, \I_n$ with $0\leq s \leq 1$. 
RRR with this normalizing matrix corresponds to a family of objectives which interpolate between RRMSE at $s=0$ and CCA at $s=1$.


% The linear RRR problem was introduced in \cite{}.

% When $\Y=\X$ and $\Sig=\I$, then the objective \eqref{eq:genrrr2} is PCA and $\V_x\x_t$ is the PCA projection with output whitening.
% Therefore, this can be viewed as a supervised PCA objective function.
% (Actually, this is exactly supervised PCA if we assume $\V_x^\top\V_x=\I_k$. Thus, we can view this as supervised PCA with output whitening.)
% When $\Sig=\C_{yy}$, the objective is related to CCA and $\V_x\x_t$ is the CCA projection for $\x_t$.

% In this work we focus on 2 cases: $\Sig=\I_n$ and $\Sig=\C_{yy}$.
% When $\Sig=\I_n$, the problem is referred to as FILL IN.
% When $\Sig=\C_{yy}$ the problem is related to CCA \cite{izenman1975reduced}.
% In fact, in this case, the projection $\V_x^\top\x_t$ is equal to the CCA projection (see Supplemental Material).

% \paragraph{Reduced Rank Regression.~} Reduced rank regression (RRR)~\cite{anderson1951estimating,izenman1975reduced}, is a variation of multi-variate linear regression where the matrix of regression weights is constrained to be low-rank. 
% Explicitly, given centered predictor and response matrices $\X$ and $\Y$, RRR is formulated as minimizing the following objective  function:
% \begin{equation}\label{eq:rrr}
%     \min_{{\bf P}\in\R^{n\times m}} \big\big\lVert\Y - {\bf P} \X \big\big\rVert^2\quad\text{subject to}\quad\text{rank}({\bf P})\le k,
% \end{equation}
% where $\P\in\R^{n\times m}$ is the matrix of regression weights and $k\le\min(m,n)$ determines the rank of the problem. This low-rank constraint can be explicitly implemented by letting $\P=\V_y \V_x^\top$ and rewriting the objective as
% \begin{equation}\label{eq:rrr_VxVy}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}} \big\big\lVert\Y - \V_y\V_x^\top \X \big\big\rVert^2.
% \end{equation}
% For any given solution to this optimization objective  $(\V_x,\V_y)$, there exists a family of solutions generated by invertible matrices $\M\in\R^{k\times k}$ given by $(\V_x\M^\top,\V_y\M^{-1})$.
% It is common to reduce this degeneracy of solutions by imposing the whitening constraint $\V_x^\top \C_{xx} \V_x=\I_k$. 
% Expanding the quadratic in \eqref{eq:rrr_VxVy}, ignoring the constant $\Y\Y^\top$ term, and using the whitening constraint, we arrive at the following objective:
% \begin{equation}\label{eq:RRR_first}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\tr\V_y^\top\V_y-2\V_x^\top \C_{xy}\V_y,\quad\text{subject to}\;\V_x^\top \C_{xx}\V_x=\I_k.
% \end{equation}
% Reduced rank regression has wide applications~\cite{rrr_book}. This is in part because it can be used as an explicit regularizer to reduce over-fitting of the responses~\cite{izenman1975reduced}. But also because it is an effective tool for dimensionality reduction~\cite{sparese_rrr} in the sense that the projection matrix $\V_x^\top \X$ is the subspace of the predictor matrix $\X$ which is maximally informative of the responses $\Y$. In this interpretation, RRR is not an algorithm for inferring the response of a system, but much like canonical correlation analysis, it is a self-supervised  algorithm where part of the data is being used to compress the rest. 

% \paragraph{Canonical correlation analysis.~} Introduced by Hotelling in 1936~\cite{hotelling1936relations}, canonical correlation analysis is a statistical tool for dimensionality reduction based on the cross-correlation of two multi-dimensional variables~\cite{cca_tutorial}.  Explicitly, given two data matrices $\X$ and $\Y$, the CCA objective is to find the subspace of $\X$ and $\Y$ such that their cross-correlation is maximized:
% \begin{align}\label{eq:CCA_lin_obj}
%     \argmax{\W_x\in\R^{m\times k},\W_y\in\R^{n\times k}}\tr\left(\W_x^\top \C_{xy}\W_y\right) ,\quad\text{subject to}\;
%     \W_x^\top\C_{xx}\W_x=\W_y^\top \C_{yy}\W_y=\I_k.
% \end{align}
% To proceed, it is convenient to use the eigenvalue formulation of CCA~(see Sec.~\ref{app:CCA_op_2_eig} of supplementary materials):
% \begin{align}\label{eq:CCA_eig_start}
%     \C_{xx}^{-1}\C_{xy}\C_{yy}^{-1}\C_{yx}\V_x=\V_x\Lam^2,\quad\text{subject to}\;\V_x^\top\C_{xx}\V_x=\I_k,
% \end{align}
% where $\Lam$ is the diagonal matrix of canonical correlations\footnote{\note{SG: this is only diagonal in the correct basis and the derivation in the appendix does not necessarily bring it into this diagonal form.}} and columns of $\V_x$ are the canonical correlation basis vectors. Multiplying on both sides by $\V_x^\top\C_{xx}$ we arrive at
% \begin{align*}
%     \V_x^\top\C_{xy}\C_{yy}^{-1}\C_{yx}\V_x=\Lam^2,
% \end{align*}
% where we have used the constraint $\V_x^\top\C_{xx}\V_x=\I_k$. We can therefore find the subspace spanned by the canonical basis elements corresponding to the highest eigenvalues as the span of the columns of the matrix $\V_x$ which maximizes the following objective.
% \begin{equation}
%     \max_{\V_x\in\R^{m\times k}} \tr\V_x^\top\C_{xy}^\top \C_{yy}^{-1}\C_{yx}\V_x,\quad\text{subject to}\;\V_x^\top \C_{xx}\V_x=\I_k.
% \end{equation}
% We can simplify this objective by introducing an auxiliary variable $\V_y$. Multiplying by an overall minus sign and switching from $\max$ to $\min$ brings us to
% \begin{equation}\label{eq:CCA_first}
%     \min_{\V_x\in\R^{m\times k}}\min_{\V_y\in\R^{n\times k}}\tr\V_y^\top\C_{yy}\V_y-2\V_x^\top\C_{xy}\V_y,\quad\text{subject to}\;\V_x^\top\C_{xx}^\top\V_x=\I_k.
% \end{equation}
% In this formulation the matrix $\V_x$ is the same as the $\W_x$ matrix in the formulation of Eq.~\eqref{eq:CCA_lin_obj}. However, while $\V_y$ and $\W_y$ span the same subspace, $\V_y$ does not satisfy the same normalization constraint, i.e. $\W_y = (\V_y^\top \C_{yy}\V_y)^{-1/2} \V_y$. For more details see supplementary materials Sec.~\ref{app:CCA_op_2_eig}.

% Comparison of the RRR and CCA objective in Eqs.~\eqref{eq:RRR_first} and ~\eqref{eq:CCA_first} demonstrates the close relationship between the two methods~\cite{cca_tutorial,rrr_book,de2012least}. In the following sections we show how these objectives can be turned into online algorithms and then into biologically plausible neural networks. 
% The derivation of the algorithm for each problem is similar, however, for clarity we will consider them separately.
